EISim: A Platform for Simulating Intelligent Edge Orchestration Solutions

To support the stringent requirements of the future intelligent and interactive applications, intelligence needs to become an essential part of the resource management in the edge environment. Developing intelligent orchestration solutions is a challenging and arduous task, where the evaluation and comparison of the proposed solution is a focal point. Simulation is commonly used to evaluate and compare proposed solutions. However, the currently existing, openly available simulators are lacking in terms of supporting the research on intelligent edge orchestration methods. To address this need, this article presents a simulation platform called Edge Intelligence Simulator (EISim), the purpose of which is to facilitate the research on intelligent edge orchestration solutions. EISim is extended from an existing fog simulator called PureEdgeSim. In its current form, EISim supports simulating deep reinforcement learning based solutions and different orchestration control topologies in scenarios related to task offloading and resource pricing on edge. The platform also includes additional tools for creating simulation environments, running simulations for agent training and evaluation, and plotting results.

==> Chapters/abbreviations.tex <==
AI      Artificial Intelligence
AP      Access Point
DAG     Directed Acyclic Graph
DDPG    Deep Deterministic Policy Gradient
DRL     Deep Reinforcement Learning
ESP     Edge Service Provider
IID     Independent and Identically Distributed
LAN     Local Area Network
MAN     Metropolitan Area Network
MAS     Multi-agent System
MEC     Multi-access Edge Computing
MI      Million Instruction
MIPS    Million Instructions per Second
TWST    Tunable Weight Spanning Tree
VM      Virtual Machine
WAN     Wide Area Network



